StepDIRECT -- A Derivative-Free Optimization Method for Stepwise Functions

In this paper, we propose the StepDIRECT algorithm for derivative-free optimization (DFO), in which the black-box objective function has a stepwise landscape. Our framework is based on the well-known DIRECT algorithm. By incorporating the local variability to explore the flatness, we provide a new criterion to select the potentially optimal hyper-rectangles. In addition, we introduce a stochastic local search algorithm performing on potentially optimal hyper-rectangles to improve the solution quality and convergence speed. Global convergence of the StepDIRECT algorithm is provided. Numerical experiments on optimization for random forest models and hyper-parameter tuning are presented to support the efficacy of our algorithm. The proposed StepDIRECT algorithm shows competitive performance results compared with other state-of-the-art baseline DFO methods including the original DIRECT algorithm.

==> sections/bayes_opt.tex <==
\section{Introduction to Bayesian Optimization}\label{sec: bayes_opt}
Bayesian optimization falls in a class of optimization algorithms called sequential model-based optimization (SMBO) algorithms. These algorithms use previous observations of the loss $f$, to determine the next (optimal) point to sample $f$
 for. The algorithm can roughly be outlined as follows.
 
 
 \begin{algorithm}[htb!]
	\caption{Bayesian Optimization}\label{alg: bayes_opt}
	\begin{algorithmic}
	\STATE \FOR{t=1,2,\ldots}
	\STATE Find $x_t$ by optimizing the acquisition function over the Gaussian Process: $x_t=\argmax_{x}u(x|\mathcal{D}_{1:t-1})$.
	\STATE Evaluate function at $x_t$: $y_t=f(x_t)$.
	\STATE Augment the data $\mathcal{D}_{1:t}=\{\mathcal{D}_{1:t-1}, (x_t, y_t)\}$
	\ENDFOR
	\end{algorithmic}
\end{algorithm}
